Bounds on Optimal Revisit Times in Persistent Monitoring Missions with a Distinct \& Remote Service Station

Persistent monitoring missions require an up-to-date knowledge of the changing state of the underlying environment. UAVs can be gainfully employed to continually visit a set of targets representing tasks (and locations) in the environment and collect data therein for long time periods. The enduring nature of these missions requires the UAV to be regularly recharged at a service station. In this paper, we consider the case in which the service station is not co-located with any of the targets. An efficient monitoring requires the revisit time, defined as the maximum of the time elapsed between successive revisits to targets, to be minimized. Here, we consider the problem of determining UAV routes that lead to the minimum revisit time. The problem is NP-hard, and its computational difficulty increases with the fuel capacity of the UAV. We develop an algorithm to construct near-optimal solutions to the problem quickly, when the fuel capacity exceeds a threshold. We also develop lower bounds to the optimal revisit time and use these bounds to demonstrate (through numerical simulations) that the constructed solutions are, on an average, at most 0.01% away from the optimum.

==> sections/comparison.tex <==
Advantages of {\prob}
\begin{itemize}
    \item Wider applicability
    \item Convenience of introducing the service time
    \item Path to solve the weighted PMP which is computationally challenging
\end{itemize}

Difference in structure
\begin{itemize}
    \item Objective
    \item Visits to the service station
\end{itemize}

Computational difficulty
\begin{itemize}
    \item Every {\prob} solution can be considered as a feasible solution for PMP (by considering the service station of {\prob} as an additional target in PMP).
    \item Therefore, {\prob} is at least as difficult as PMP to solve.
    \item In \cite{hari20tro}, we solve PMP. Here, we set to characterize the structure of optimal solutions to {\prob}.
\end{itemize}







% ************
\cite{hari20tro} considers a related problem referred to as the persistent monitoring problem (PMP). In PMP, the service station is located at one of the targets. The rationale behind this positioning is to increase the time spent on monitoring the environment by reducing the travel time between the service station and the targets. However, this restricts the suitability of PMP to only civilian applications in which the targets are accessible for vehicle servicing. On the other hand, {\prob} does not place any restrictions on the depot location, and hence is suitable for a broader range of applications (for example, {\prob} is even applicable in military applications in which targets are not accessible).
% \cite{hari20tro} considers a related problem referred to as the persistent monitoring problem (PMP), in which the service station is positioned at one of the targets. This positioning facilitates the environment to be monitored for a longer duration by eliminating the travel time between targets and the service station. However, this restricts the suitability of PMP to only civilian applications in which the targets are accessible for vehicle servicing. One the other hand, {\prob} does not place any restrictions on the location of the service station and therefore has a broader applicability (for example, it is also suitable for military applications where the targets are not accessible).

From a technical point of view, {\prob} has the following subtle differences from PMP: 1) firstly, in each servicing cycle, {\prob} allows exactly one visit to the service station, whereas PMP allows multiple visits to the target at which the service station is located; 2) secondly, the revisit time of the service station is not factored in the objective for {\prob}, but is a part of the objective for PMP. These subtle differences change the character of the problem and the characterization of optimal routes and is a subject of investigation in this paper.

Besides, solving {\prob} also helps tackling an important generalization of the PMP, in which certain targets are weighted differently compared to the rest; this generalization is referred to as the weighted PMP. The service station in {\prob} can be considered as an additional target with a lower priority (and thereby visited only once). Therefore, by characterizing optimal {\prob} solutions and by introducing weighted targets one at a time, one can potentially solve the weighted PMP. 

% {\color{blue} {\prob} has a capability of accounting for a-priori given arbitrary dwell times and servicing times}

% A variant of the {\prob} in which the service station is located at one of the targets has been considered in \cite{hari20tro}. This variant, referred to as the PMP, ensures that the environment is monitored for a longer duration by eliminating the travel time between the targets and the service station.
% However, this restricts the suitability of PMP to only civilian applications in which the targets are accessible for vehicle servicing. In {\prob}, 
% Suitability of PMP is restricted to only civilian applications in which the targets are accessible for vehicle servicing. %, whereas, {\prob} relaxes this restriction and widens its scope of applicability.

% From a technical point of view, PMP differs from PMP-D since the objective is subtly different - the revisit time to depot is not factored in the objective for PMP-D, but is accounted for in PMP. This subtle difference changes the character of the problem and the characterization of optimal routes and is a subject of investigation in this paper. 

% Similar to {\prob}, it is computationally challenging to find optimal PMP solutions, and the computation time increases rapidly with $k$. However, in \cite{hari20tro}, we characterized the structure of optimal PMP solutions and developed results that lead to a swift computation of these solutions. The computation time improved from tens of hours to a mere fraction of a second on a standard laptop for instances with upto 30 targets.
% Solutions to {\prob} differ from those to PMP, as the former have exactly one visit to the depot in each servicing cycle, whereas the latter allows multiple visits to the target at which the depot is located in a single servicing cycle. 

% Every feasible {\prob} solution can be considered as a feasible solution to a PMP. This makes {\prob} computationally at least as difficult as PMP.
Nonetheless, both {\prob} and PMP are computationally challenging (NP-Hard) and the computation time for finding optimal solutions increases rapidly with $k$. In \cite{hari20tro}, we characterized the structure of optimal PMP solutions and developed results that lead to a swift computation of these solutions. The computation time improved from tens of hours to a mere fraction of a second on a standard laptop for instances with upto 30 targets. Similarly, in the current paper, we set out to characterize the structure of optimal solutions for {\prob} by providing tight bounds on the optimal revisit times for different values of $k$. With these bounds, we compute either optimal (in some cases) or near-optimal solutions to the problem swiftly. 


==> sections/notes.tex <==
Dwells times can be easily introduced to suit applications in which the time spent by agents at the targets is of importance.
